DiffuCOMET: Contextual Commonsense Knowledge Diffusion

Inferring contextually-relevant and diverse commonsense to understand narratives remains challenging for knowledge models. In this work, we develop a series of knowledge models, DiffuCOMET, that leverage diffusion to learn to reconstruct the implicit semantic connections between narrative contexts and relevant commonsense knowledge. Across multiple diffusion steps, our method progressively refines a representation of commonsense facts that is anchored to a narrative, producing contextually-relevant and diverse commonsense inferences for an input context. To evaluate DiffuCOMET, we introduce new metrics for commonsense inference that more closely measure knowledge diversity and contextual relevance. Our results on two different benchmarks, ComFact and WebNLG+, show that knowledge generated by DiffuCOMET achieves a better trade-off between commonsense diversity, contextual relevance and alignment to known gold references, compared to baseline knowledge models.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/deleted_tables.tex <==

\begin{table*}[t]
\centering
\resizebox{1.0\textwidth}{!}{
\smallskip\begin{tabular}{lccccccccccc}
\hline
\multirow{2}*{\textbf{Model}} & \multirow{2}*{\textbf{\# Facts}}  & \multicolumn{5}{c}{\textbf{Clustering \wrt{} Word-Level Edit Distance}} & \multicolumn{5}{c}{\textbf{Clustering \wrt{} Embedding Euclidean Distance}}\\
            \cmidrule(lr){3-7} \cmidrule(lr){8-12}
 &  & \textbf{\# Clusters} & \textbf{Diversity}  & \textbf{Relevance} & \textbf{Alignment} & \textbf{F1} & \textbf{\# Clusters} & \textbf{Diversity}  & \textbf{Relevance} & \textbf{Alignment} & \textbf{F1} \\
\hline
Greedy        & 2.48  & 1.08 & 43.54 & 32.04 & 31.98 & 32.01 & 1.09 & 43.95 & 32.11 & 48.59 & 38.67 \\
Sampling   & 10.00 & 5.59 & 55.90 & 39.20 & 46.03 & 42.34 & 5.64 & 56.40 & 38.93 & 64.51 & 48.56 \\  % Sampling-10
% Sampling-10   & 10.00 & 5.59 & 55.90 & 39.20 & 46.03 & 42.34 & 5.64 & 56.40 & 38.93 & 64.51 & 48.56 \\
% Sampling-15   & 15.00 & 7.64 & 50.93 & 37.18 & 49.78 & 42.57 & 7.82 & 52.13 & 36.86 & 68.00 & 47.81 \\
Beam       & 15.00 & 3.48 & 23.20 & 41.46 & 48.04 & 44.51 & 3.97 & 26.47 & 42.88 & 63.14 & 51.07 \\  % Beam-15
% Beam-10       & 10.00 & 2.63 & 26.30 & 38.30 & 44.96 & 41.36 & 2.83 & 28.30 & 38.87 & 59.58 & 47.05 \\
% Beam-15       & 15.00 & 3.48 & 23.20 & 41.46 & 48.04 & 44.51 & 3.97 & 26.47 & 42.88 & 63.14 & 51.07 \\
\midrule
\diffucomet-Fact   & 13.40 & 4.74 & 35.37 & 59.75 & 54.07 & 56.77 & 5.85 & 43.66 & 60.32 & \textbf{73.38} & 66.21 \\
~~~- Joint-Train & 3.64  & 2.05 & \textbf{56.32} & \textbf{73.01} & 42.54 & 53.76 & 2.09 & \textbf{57.42} & \textbf{73.19} & 56.84 & 63.99 \\
\diffucomet-Entity & 10.08 & 4.51 & 44.74 & 62.27 & \textbf{54.61} & \textbf{58.19} & 5.24 & 51.98 & 61.77 & 71.54 & \textbf{66.30} \\
\midrule
Gold          & 10.55 & 5.64 & 53.46 & 81.06 & - & - & 5.64 & 53.46 & 80.90 & - & - \\
\hline
\end{tabular}
}
\caption{Clustering-based evaluation results of contextual knowledge generation on models with BART (base) backbone, tested on the ROCStories portion of \comfact{}. Best results (excluding Gold references) are in bold. \ab{I would just pick one of these distance functions for the main result (maybe have a table for the other one in the appendix? Then put Table 2 with the raw metrics in the main table. I'm not sure there's much benefit to putting both BART-base and BART-large results in the main paper.}}
\label{tab:results_cluster_base}
\end{table*}


\begin{table}[t]
\centering
\resizebox{1.0\columnwidth}{!}{
\smallskip\begin{tabular}{lcccc}
\hline
\textbf{Model} & \textbf{Distinct-4}  & \textbf{BLEU} & \textbf{METEOR} & \textbf{ROUGE-L} \\
\hline
Greedy        & \textbf{99.90} & 8.70 & 40.49 & 44.43 \\
Sampling   & 85.29 & 7.16 & 37.78 & 39.20 \\ % Sampling-10
% Sampling-10   & 85.29 & 7.16 & 37.78 & 39.20 \\
% Sampling-15   & 81.57 & 8.24 & 38.35 & 40.13 \\
Beam       & 45.21 & 11.51 & 42.04 & 42.91 \\  % Beam-15
% Beam-10       & 50.32 & 12.25 & 42.23 & 43.53 \\
% Beam-15       & 45.21 & 11.51 & 42.04 & 42.91 \\
\midrule
\diffucomet-Fact   & 57.87 & 12.09 & \textbf{46.43} & \textbf{47.13} \\
\diffucomet-Entity & 70.02 & \textbf{14.25} & 43.34 & 45.08 \\
\midrule
Gold          & 80.45 & - & - & - \\
\hline
\end{tabular}
}
\caption{Evaluation results of natural language generation metrics on models with BART (base) backbone, tested on the ROCStories portion of \comfact{}.}
\label{tab:results_nlg_base}
\end{table}


\begin{table*}[t]
\centering
\resizebox{1.0\textwidth}{!}{
\smallskip\begin{tabular}{@{~}lcc@{~~}c@{~~~}c@{~~~}c@{~~~}cc@{~~~}c@{~~~}c@{~~~}c@{~~~}c@{~}}
\hline
\multirow{2}*{\textbf{Model}} & \multirow{2}*{\textbf{\# Facts}}  & \multicolumn{5}{c}{\textbf{Clustering \wrt{} Word-Level Edit Distance}} & \multicolumn{5}{c}{\textbf{Clustering \wrt{} Embedding Euclidean Distance}}\\
            \cmidrule(lr){3-7} \cmidrule(lr){8-12}
 &  & \textbf{\# Clusters} & \textbf{Diversity}  & \textbf{Relevance} & \textbf{Alignment} & \textbf{F1} & \textbf{\# Clusters} & \textbf{Diversity}  & \textbf{Relevance} & \textbf{Alignment} & \textbf{F1} \\
\hline
% Greedy-BART & 2.20  & 1.38 & \textbf{62.73} & 60.45 & 36.11 & 45.21 & 1.37 & \textbf{62.27} & 60.22 & 52.31 & 55.99 \\
% Greedy-\comet{} & 1.96 & 1.14 & 58.16 & 61.27 & 34.76 & 44.36 & 1.19 & 60.71 & 61.42 & 50.64 & 55.51 \\
Beam-BART  & 15.00 & 4.17 & 27.80 & 64.18 & 53.66 & 58.45 & 4.60 & 30.67 & 64.35 & 71.35 & 67.67 \\ % Beam-15
Beam-\comet{} & 15.00 & 4.78 & 31.87 & 64.91 & 54.77 & 59.41 & 5.09 & 33.93 & 65.03 & 71.64 & 68.18 \\ % Beam-15
    % & Sampling-10 & 10.00 & 6.68 & \textbf{66.80} & 56.09 & 52.10 & 54.02 & 6.40 & \textbf{64.00} & 56.68 & 73.86 & 64.14 \\
    % & Sampling-15   & 15.00 & 8.89 & 59.27 & 56.24 & 55.18 & 55.70 & 8.56 & 57.07 & 56.57 & 76.30 & 64.97 \\
    % & Beam-10       & 10.00 & 3.32 & 33.20 & 64.94 & 50.72 & 56.96 & 3.51 & 35.10 & 64.37 & 69.14 & 66.67 \\
    % & Beam-15       & 15.00 & 4.17 & 27.80 & 64.18 & 53.66 & 58.45 & 4.60 & 30.67 & 64.35 & 71.35 & 67.67 \\
    % \cmidrule(lr){2-13}
% \midrule
% \multirow{1}*{\comet{}-} & Greedy & 1.96 & 1.14 & 58.16 & 61.27 & 34.76 & 44.36 & 1.19 & 60.71 & 61.42 & 50.64 & 55.51 \\
% \multirow{1}*{BART} & Beam       & 15.00 & 4.78 & 31.87 & 64.91 & 54.77 & 59.41 & 5.09 & 33.93 & 65.03 & 71.64 & 68.18 \\ % Beam-15
    % & Sampling-10 & 10.00 & 6.45 & 64.50 & 56.79 & 53.36 & 55.02 & 6.30 & 63.00 & 56.60 & 73.64 & 64.01 \\
    % & Sampling-15   & 15.00 & 8.52 & 56.80 & 55.78 & \textbf{58.99} & 57.34 & 8.39 & 55.93 & 56.19 & \textbf{77.97} & 65.31 \\
    % & Beam-10       & 10.00 & 3.78 & 37.80 & 64.62 & 53.45 & 58.51 & 3.89 & 38.90 & 64.73 & 70.65 & 67.56 \\
    % & Beam-15       & 15.00 & 4.78 & 31.87 & 64.91 & 54.77 & 59.41 & 5.09 & 33.93 & 65.03 & 71.64 & 68.18 \\
% \midrule
Grapher & 5.08  & 1.75 & 34.45 & \textbf{67.82} & 33.07 & 44.46 & 2.60 & \textbf{51.18} & \textbf{68.29} & 40.58 & 50.91 \\
\midrule
\diffucomet-Fact   & 12.88 & 4.47 & 34.55 & 65.82 & 54.18 & 59.44 & 5.24 & 40.68 & 65.64 & 71.65 & 68.51 \\
\diffucomet-Entity & 12.89 & 5.09 & \textbf{39.49} & 67.00 & \textbf{58.22} & \textbf{62.30} & 5.67 & 43.99 & 66.39 & \textbf{74.38} & \textbf{70.16}  \\
\midrule
      Gold       & 10.55 & 5.64 & 53.46 & 81.06 & - & - & 5.64 & 53.46 & 80.90 & - & - \\
\hline
\end{tabular}
}
\caption{Clustering-based evaluation results on models with large-scale backbones, tested on the ROCStories portion of \comfact{}. Best results (excluding Gold references) are in bold. Greedy/Beam-BART/\comet{} denotes the greedy / beam search baseline model fine-tuned from BART (large) / \comet{}-BART backbone, respectively. \ab{I would just pick one of these distance functions for the main result (maybe have a table for the other one in the appendix? Then put Table 4 with the raw metrics in the main table.}}
\label{tab:results_cluster_large}
\end{table*}


\begin{table}[t]
\centering
\resizebox{1.0\columnwidth}{!}{
\smallskip\begin{tabular}{@{~}lc@{~~~}c@{~~~}c@{~~~}c@{~}}
\hline
\textbf{Model} & \textbf{Distinct-4}  & \textbf{BLEU} & \textbf{METEOR} & \textbf{ROUGE-L} \\
\hline
% Greedy-BART & \textbf{93.01} & 9.12 & 43.98 & 46.26 \\
% Greedy-\comet{} & 65.95 & 18.01 & \textbf{52.32} & \textbf{54.96} \\
Beam-BART & 43.73 & 13.11 & 47.70 & 46.35 \\ % Beam-15
Beam-\comet{} & 47.27 & 16.97 & 47.39 & 47.19 \\ % Beam-15
    % & Sampling-10 & 86.33 & 9.89 & 43.85 & 43.69 \\
    % & Sampling-15   & 81.56 & 9.47 & 43.28 & 43.15 \\
    % & Beam-10       & 47.03 & 15.02 & 48.56 & 48.15 \\
    % & Beam-15       & 43.73 & 13.11 & 47.70 & 46.35 \\
    % \cmidrule(lr){2-6}
    % & \diffucomet-Fact   & 52.46 & 15.98 & 50.06 & 51.44 \\
    % & \diffucomet-Entity & 63.49 & 17.01 & 47.61 & 48.40 \\
% \midrule
% \multirow{1}*{\comet{}-} & Greedy & 65.95 & 18.01 & \textbf{52.32} & \textbf{54.96} \\
% \multirow{1}*{BART} & Beam       & 47.27 & 16.97 & 47.39 & 47.19 \\ % Beam-15
    % & Sampling-10 & 83.29 & 13.35 & 44.77 & 45.80 \\
    % & Sampling-15   & 79.01 & 12.69 & 44.43 & 45.58 \\
    % & Beam-10       & 51.13 & \textbf{19.89} & 50.14 & 50.48 \\
    % & Beam-15       & 47.27 & 16.97 & 47.39 & 47.19 \\
% \midrule
Grapher & \textbf{67.83}  & 1.40 & 23.96 & 27.21 \\
\midrule
\diffucomet-Fact   & 52.46 & 15.98 & \textbf{50.06} & \textbf{51.44} \\
\diffucomet-Entity & 63.49 & \textbf{17.01} & 47.61 & 48.40 \\
\midrule
     Gold     & 80.45 & - & - & - \\
\hline
\end{tabular}
}
\caption{Evaluation results of natural language generation metrics on models with large-scale backbones, tested on the ROCStories portion of \comfact{}. Model notations are same as Table~\ref{tab:results_cluster_large}.}
\label{tab:results_nlg_large}
\end{table}

